Differentially Private Kernel Inducing Points using features from ScatterNets (DP-KIP-ScatterNet) for Privacy Preserving Data Distillation

Data distillation aims to generate a small data set that closely mimics the performance of a given learning algorithm on the original data set. The distilled dataset is hence useful to simplify the training process thanks to its small data size. However, distilled data samples are not necessarily privacy-preserving, even if they are generally humanly indiscernible. To address this limitation, we introduce differentially private kernel inducing points (DP-KIP) for privacy-preserving data distillation. Unlike our original intention to simply apply DP-SGD to the framework of KIP, we find that KIP using infinitely-wide convolutional neural tangent kernels (conv-NTKs) performs better compared to KIP using fully-connected NTKs. However, KIP with conv-NTKs, due to its convolutional and pooling operations, introduces an unbearable computational complexity, requiring hundreds of V100 GPUs in parallel to train, which is impractical and more importantly, such computational resources are inaccessible to many. To overcome this issue, we propose an alternative that does not require pre-training (to avoid a privacy loss) and can well capture complex information on images, as those features from conv-NKTs do, while the computational cost is manageable by a single V100 GPU. To this end, we propose DP-KIP-ScatterNet, which uses the wavelet features from Scattering networks (ScatterNet) instead of those from conv-NTKs, to perform DP-KIP at a reasonable computational cost. We implement DP-KIP-ScatterNet in -- computationally efficient -- JAX and test on several popular image datasets to show its efficacy and its superior performance compared to state-of-the art methods in image data distillation with differential privacy guarantees.

==> tables/dp_comparison_image.tex <==
\begin{table*}
    \caption{\textbf{Left:} Test accuracy of ConvNet downstream classifier trained on synthetic/distilled data with $\delta=10^{-5}$. \textbf{Right:} Test accuracy of ConvNet downstream classifier trained with  fixed $\epsilon=10$ and $\delta=10^{-5}$ and varying the number of distilled samples per class. 
    % In \citet{DPSGD_GM}, they created $20$ distilled images per class. 
    In concurrent work \cite{anonymous2023differentially}, the test accuracy on the same classifier tested on $50$ MNIST distilled samples created at $\epsilon=6.12$ and $\delta=10^{-5}$
    is $97.35\%$; that on $50$  Fashion-MNIST distilled samples  created at $\epsilon=5.45$ and $\delta=10^{-5}$
    is $82.72\%$
    }
    \label{tab:dpmethods_img_comp}
\begin{minipage}{\columnwidth}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c |cc | cc}
\toprule
&  \multicolumn{2}{|c|}{MNIST} & \multicolumn{2}{|c}{FASHION} \\
& $\epsilon=1$  & $\epsilon=10$ & $\epsilon=1$  & $\epsilon=10$\\ \hline
DP-CGAN & - & 52.5 & - & 50.2 \\
G-PATE & 58.8 & 80.9 & 58.1 & 69.3 \\
DataLens & 71.2 & 80.7 & 64.8 & 70.6\\
GS-WGAN & - & 84.9 & - & 63.1 \\
DP-MERF & 72.7 & 85.7 & 61.2 & 72.4 \\
DP-Sinkhorn & - & 83.2 & - & 71.1 \\
\midrule
 \citet{DPSGD_GM}  & & & \\
(20 Imgs/Class)  & 80.9 & 95.6 & 70.2 & 77.7 \\
DP-KIP FC & &\\
(10 Imgs/Class) & 93.53 &  95.39 & 87.7 & 89.1\\
DP-KIP FC & &\\
(20 Imgs/Class) & \textbf{97.78} & \textbf{97.96} & \textbf{88.3}  & \textbf{90.2} \\
DP-KIP ScatterNet & &\\
(10 Imgs/Class) &  &   &  & \\
DP-KIP ScatterNet & &\\
(20 Imgs/Class) &  &  &  &  \\
\bottomrule
    \end{tabular}}
\end{minipage}\hfill % maximize the horizontal separation
\begin{minipage}{\columnwidth}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c |ccc |ccc}
\toprule
&  \multicolumn{3}{|c|}{MNIST} & \multicolumn{3}{|c}{FASHION} \\

Imgs/Class & 10 & 20 & full & 10 & 20 & full \\
\hline
Real & 93.6 & 95.9 & 99.6 & 74.4 & 77.4 & 93.5 \\
DP-SGD & - & - & 96.5  &  - & - & 82.9 \\
\hline
DP-CGAN & 57.4 & 57.1 & 52.5 & 51.4 & 53.0 & 50.2 \\
GS-WGAN & 83.3 & 85.5 & 84.9 & 58.7 & 59.5 & 63.1 \\

DP-MERF & 80.2 & 83.2 & 85.7 &  66.6 & 67.9 & 72.4 \\ 
\midrule
 \citet{DPSGD_GM} & 94.9 & 95.6 & - & 75.6 & 77.7 & - \\
DP-KIP FC & \textbf{95.39} & \textbf{97.96} & - & \textbf{89.1} &  \textbf{90.2} & -\\
DP-KIP ScatterNet &  &  & - &  &  & -\\
\bottomrule
\end{tabular}}
  \end{minipage}
\end{table*}

==> tables/dpkip_hyperparam_tab_data.tex <==
% \begin{wraptable}{r}{0.5\textwidth}
\begin{table}[!h]
\caption{DP-KIP hyper-parameters settings for tabular datasets with $\epsilon=1$ and $\delta=10^{-5}$}
\label{tab:tab_data_description}
\vskip 0.1in
\centering
\scalebox{0.85}{
\begin{tabular}{l c c c c c c}
\toprule
% \tabhead{dataset} & \tabhead{$\#$ samps}  & \tabhead{$\#$ classes} & \tabhead{ $\#$ features}  \\
dataset & batch rate & undersampled rate & epochs & learning rate & $C$ & $\lambda$  \\
\midrule
isolet &   \\
covtype &  \\
epileptic & 0.01 & 0.01 & 10 & $10^{-3}$ & 0.1 & $10^{-6}$\\
credit & 0.01 & 0.04 & 10 & $10^{-4}$ & $10^{-3}$ & $10^{-6}$ \\
cervical \\
census & \\
adult &\\
intrusion & \\
\bottomrule\\
\end{tabular}

}
  \vspace{-0.5cm}
\end{table}
% \end{wraptable}


